Critical Behavioral Traits Foster Peer Engagement in Online Mental Health Communities

Online Mental Health Communities (OMHCs), such as Reddit, have witnessed a surge in popularity as go-to platforms for seeking information and support in managing mental health needs. Platforms like Reddit offer immediate interactions with peers, granting users a vital space for seeking mental health assistance. However, the largely unregulated nature of these platforms introduces intricate challenges for both users and society at large. This study explores the factors that drive peer engagement within counseling threads, aiming to enhance our understanding of this critical phenomenon. We introduce BeCOPE, a novel behavior encoded Peer counseling dataset comprising over 10,118 posts and 58,279 comments sourced from 21 mental health-specific subreddits. The dataset is annotated using three major fine-grained behavior labels: (a) intent, (b) criticism, and (c) readability, along with the emotion labels. Our analysis indicates the prominence of ``self-criticism'' as the most prevalent form of criticism expressed by help-seekers, accounting for a significant 43% of interactions. Intriguingly, we observe that individuals who explicitly express their need for help are 18.01% more likely to receive assistance compared to those who present ``surveys'' or engage in ``rants.'' Furthermore, we highlight the pivotal role of well-articulated problem descriptions, showing that superior readability effectively doubles the likelihood of receiving the sought-after support. Our study emphasizes the essential role of OMHCs in offering personalized guidance and unveils behavior-driven engagement patterns.

==> Tables/OMHC_post_sample.tex <==
% \begin{table}[]
% \begin{tabular}{|p{0.06\textwidth}|p{0.14\textwidth}|p{0.32\textwidth}|p{0.13\textwidth}|p{0.05\textwidth}|p{0.1x\textwidth}|p{0.1\textwidth}|}
% \hline
% sub\_id & title & body & author  &score & comments & created  \\ \hline
% eiu2by & Does it look like PTSD?                 & So I’m 17 F, and I think I might have PTSD and will very probably try and consult a therapist about it sooner than later.So, I’ve never liked to drive, I’ve always been scared and stressed about it and thought I wasn’t ever liking the feeling of controlling a deadly weapon... & arichou04     & 1 & 1 & 2020-01-02 5:38:15  \\ \hline
% eivvsf & Should I push myself?                   & I have been having the same conflict with my partner for awhile now.  4 years ago I was with someone who assaulted me with a kitchen knife and strangled me until I blacked out. That was just what ended our relationship but it had been 2 years of physical, sexual and emotional abuse. I have terrible flashbacks, and triggers, and they usually go on through the night. I live in the basement of my mom's house now; it is the only place I feel safe enough to live...                              & hannah2lovely & 1 & 3 & 2020-01-02 8:57:46  \\ \hline
% eix3mj & Advice - working with PTSD              & hey guys im wondering if you can help ive been suffering with PTSD which i was not asked about when joining my organisation (ie they didnt ask me about health issues). its really affected my work lately, lots of avoidance on certain tasks and going over the top of others. i havent been performing. i have been signed off now by my doctor and am wondering what to do. can you get fired if you weren't well? or do you have to declare before starting? & doddle30      & 1 & 5 & 2020-01-02 11:26:02 \\ \hline
% \end{tabular}
% \caption{A sample of posts from the OMHC dataset}
% \end{table}




% \begin{table}[]\centering
% \footnotesize
% % \begin{tabular}{l|rrrrr}\toprule
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|p{10em}|p{20em}|c|c|c|c}\toprule

% S.ID & Title & Body & Author & Score & Comm & Date \\
% \cmidrule{1-7}


% eiu2by & Does it look like PTSD?                 & So I’m 17 F, and I think I might have PTSD and will very probably try and consult a therapist about it sooner than later.So, I’ve never liked to drive, I’ve always been scared and stressed about it and thought I wasn’t ever liking the feeling of controlling a deadly weapon... & arichou04     & 1 & 1 & 2020-01-02 5:38:15  \\ 
% \cmidrule{1-7}

% eivvsf & Should I push myself?                   & I have been having the same conflict with my partner for awhile now.  4 years ago I was with someone who assaulted me with a kitchen knife and strangled me until I blacked out. That was just what ended our relationship but it had been 2 years of physical, sexual and emotional abuse. I have terrible flashbacks, and triggers, and they usually go on through the night. I live in the basement of my mom's house now; it is the only place I feel safe enough to live...                              & hannah2lovely & 1 & 3 & 2020-01-02 8:57:46  \\
% \cmidrule{1-7}
% eix3mj & Advice - working with PTSD              & hey guys im wondering if you can help ive been suffering with PTSD which i was not asked about when joining my organisation (ie they didnt ask me about health issues). its really affected my work lately, lots of avoidance on certain tasks and going over the top of others. i havent been performing. i have been signed off now by my doctor and am wondering what to do. can you get fired if you weren't well? or do you have to declare before starting? & doddle30      & 1 & 5 & 2020-01-02 11:26:02 \\ 
% \cmidrule{1-7}

% \end{tabular}}
% \caption{A sample of posts from the \peerData\ dataset. Each post contains \textit{title} and \textit{body} along with metadata including \textit{Subreddit-ID (S.ID), author, score, comments, date}. \hl{Do we need these metadata? Also, I think Table 1 and 2 can be clubbed together.}}
% \label{sample_posts}
% \end{table}



% \begin{table}[]\centering
% \footnotesize
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c p{50em}}\toprule
% \multicolumn{2}{c}{Post 1: Interactive Engagement}\\
% \cmidrule{1-2}
% \multicolumn{2}{p{\dimexpr\linewidth-2\tabcolsep\relax}}{\textbf{Post:} Over text. I’m not confident enough to do it in real life to their face. I’m scared of what this person will say. If I’ll get 10x more abuse hurled at me like usual. I can’t help but assume everyone will be like her.}\\
% &$\hookrightarrow$ \textit{Peer1: This inspires me.}\\
% &$\hookrightarrow$ \textit{Peer2: You are worth it! Someone who acts like this will never see your worth but it is still there. You are an amazing person and most people would t make it through like you have!}\\
% &$\hookrightarrow$ \textit{Peer 3: Wow, setting those boundaries is so scary it took me so long to even begin to be able to. It has such an amazing effect on your mind to know you didn't back down, in breaking down all the fear abuse has created in us over the years and starting the process of being safe enough to trust people again. You did amazingly whatever the outcome, that you did it is all that matters. Well done.}\\
% &\hspace{5mm}$\hookrightarrow$ \textit{OP: It’s terrifying to set boundaries, but it’s necessary. Like ripping off an old bandaid.}\\
% &\hspace{10mm}$\hookrightarrow$ \textit{Peer 3: Definitely, I still find it really hard with some people}\\
% \cmidrule{1-2}

% \multicolumn{2}{c}{Post 2: Non-Interactive Engagement}\\
% \cmidrule{1-2}
% \multicolumn{2}{p{\dimexpr\linewidth-2\tabcolsep\relax}}{\textbf{Post:} Hi I'm 13 and I think I'm depressed and idk how I can get help. My mom probably wouldn't care and idk I'm worried my school would make people think I'm weird of something. Idk, this stuff is too hard lol}\\
% &$\hookrightarrow$ \textit{Peer 1: Your school counselor could be a good starting point. When I first attempted to get help, I wrote a letter to my mentor about it.}\\
% &$\hookrightarrow$ \textit{Peer2: Talk with some of your teachers.}\\
% \cmidrule{1-2}
% \multicolumn{2}{c}{Post 3: Isolated Engagement}\\
% \cmidrule{1-2}
% \multicolumn{2}{p{\dimexpr\linewidth-2\tabcolsep\relax}}{\textbf{Post:} Hi there everyone, remember that tonight and many other nights in they year will have the shiniest trigger of them all, fireworks. Bit of advice on how to handle them: Don't ask people to stop them (it won't help the situation and you'll probably regret asking later on), if you absolutely can't handle it then put on some headphones and listen to something catchy (helped me get through some rough times in Afghan), and for the long term, try to get used to being around them. As long as I'm aware they're coming I can condition myself to not acknowledge them, thanks to exposure therapy. Remember to keep someone available to contact if needed and get something to eat and drink. Stay safe and happy new year.}\\
% &$\hookrightarrow$ \textit{No Comments}\\

% \bottomrule
% \end{tabular}}
% \caption{A sample of posts and comments from each of the engagement categories in the \peerData\ dataset. In the \peer\ counseling method, the original poster (OP) initiates a post, and peers interact via comments. In \peerData, posts are categorized into three engagement categories, namely a) Interactive -- where both OP and peers interact, b) Non-Interactive -- where only peers interact, and c) Isolated -- no interaction}
% \label{sample_posts}
% \end{table}




\begin{table}[]\centering
% \footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{1em}p{50em}}\toprule
\rowcolor{cyan!20} \multicolumn{2}{c}{\bf Post 1: Interactive Engagement}\\
\cmidrule{1-2}
\multicolumn{2}{p{52em}}{\textbf{Post:} Over text. I’m not confident enough to do it in real life to their face. I’m scared of what this person will say. If I’ll get 10x more abuse hurled at me like usual. I can’t help but assume everyone will be like her.}\\
&$\hookrightarrow$ \textit{\textbf{Peer 1:} This inspires me.}\\
&$\hookrightarrow$ \textit{\textbf{Peer 2:} You are worth it! Someone who acts like this will never see your worth but it is still there. You are an amazing person and most people would t make it through like you have!}\\
&$\hookrightarrow$ \textit{\textbf{Peer 3:} Wow, setting those boundaries is so scary it took me so long to even begin to be able to. It has such an amazing effect on your mind to know you didn't back down, in breaking down all the fear abuse has created in us over the years and starting the process of being safe enough to trust people again. You did amazingly whatever the outcome, that you did it is all that matters. Well done.}\\
&\hspace{5mm}$\hookrightarrow$ \textit{\textbf{OP:} It’s terrifying to set boundaries, but it’s necessary. Like ripping off an old bandaid.}\\
&\hspace{10mm}$\hookrightarrow$ \textit{\textbf{Peer 3:} Definitely, I still find it really hard with some people}\\
\cmidrule{1-2}

\rowcolor{cyan!20} \multicolumn{2}{c}{\bf Post 2: Non-Interactive Engagement}\\
\cmidrule{1-2}
\multicolumn{2}{p{52em}}{\textbf{Post:} Hi I'm 13 and I think I'm depressed and idk how I can get help. My mom probably wouldn't care and idk I'm worried my school would make people think I'm weird of something. Idk, this stuff is too hard lol}\\
&$\hookrightarrow$ \textit{\textbf{Peer 1:} Your school counselor could be a good starting point. When I first attempted to get help, I wrote a letter to my mentor about it.}\\
&$\hookrightarrow$ \textit{\textbf{Peer 2:} Talk with some of your teachers.}\\
\cmidrule{1-2}
\rowcolor{cyan!20} \multicolumn{2}{c}{\bf Post 3: Isolated Engagement}\\
\cmidrule{1-2}
\multicolumn{2}{p{52em}}{\textbf{Post:} Hi there everyone, remember that tonight and many other nights in they year will have the shiniest trigger of them all, fireworks. Bit of advice on how to handle them: Don't ask people to stop them (it won't help the situation and you'll probably regret asking later on), if you absolutely can't handle it then put on some headphones and listen to something catchy (helped me get through some rough times in Afghan), and for the long term, try to get used to being around them. As long as I'm aware they're coming I can condition myself to not acknowledge them, thanks to exposure therapy. Remember to keep someone available to contact if needed and get something to eat and drink. Stay safe and happy new year.}\\
&$\hookrightarrow$ \textit{No Comments}\\
\bottomrule \\
\end{tabular}}
\caption{A sample of posts and comments from each of the engagement categories in the \peerData\ dataset. In the \peer\ counseling method, the original poster (OP) initiates a post, and peers interact via comments. In \peerData, posts are categorized into three engagement categories, namely (a) Interactive -- where both OP and peers interact, (b) Non-interactive -- where only peers interact, and (c) Isolated -- no interaction.}
\label{sample_posts}
\end{table}

==> Tables/annotation_criticizm.tex <==
\begin{table}[]\centering
\footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{40em}|p{7em}} \toprule

Post & Label\\
\cmidrule{1-2}
I’ve taken lexapro and Effexor for anxiety, and neither have helped. If anything my anxiety is worse. The only med that has helped me with anxiety is klonopin, however I switched psychiatrists and my new one took me off of it because I am a minor (17) and it is highly addictive. Should I try to get prescribed it again? My anxiety is so bad that maybe it’s worth getting an addiction for. & \multirow{4}{7em}{\centering No Criticism} \\
\cmidrule{1-2}
My mental illnesses dictate so much of my daily life that I genuinely don't know what life would be like without them. I've wasted so much of what should have been very formative years for me caught up in being sad or anxious or hating myself all the time that I feel like I never got the chance to develop a personality separate from my illnesses. That makes me terrified of recovery, feeling like my illnesses are a part of me to my very cor \hl{incomplete sentence?} & \multirow{4}{7em}{\centering Self criticism} \\
\cmidrule{1-2}
I'm in the highway, my dad is driving, he is mad, really mad.He has done this before, but before it was just me, he is treating to kill us, I don't know what to do, I don't want to die like this, I don't want to die by his (obscenity) hands, I'll rather a painful illness that him taking my life, he doesn't deserve my life.Please help, I'm scared. & \multirow{4}{7em}{\centering Others' criticism with reason} \\
\cmidrule{1-2}
First of all  you're all weak. PTSD is a joke. Almost laughable as 9/11 and The Holocaust being real. You're all actors. You're all failures and should've been aborted! You waste of space lame obscenities\{{]}\}. None of you all could ever have your own place cause you're all too slobbish and would be kicked out for your pure incompetence and lack of life. & \multirow{4}{7em}{\centering Others' criticism without reason} \\                                
% \cmidrule{1-8}
% \bottomrule{1-3}
\bottomrule
\end{tabular}}
\caption{Annotations for Criticism}
\label{criticism_example}
\end{table}

% \begin{table}[]\centering
% \footnotesize
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|c|p{40em}}\toprule

% Label & Meaning & Example\\
% \cmidrule{1-3}
% 0 & No Criticism & I’ve taken lexapro and Effexor for anxiety, and neither have helped. If anything my anxiety is worse. The only med that has helped me with anxiety is klonopin, however I switched psychiatrists and my new one took me off of it because I am a minor (17) and it is highly addictive. Should I try to get prescribed it again? My anxiety is so bad that maybe it’s worth getting an addiction for.\\
% \cmidrule{1-3}
% 1a & Self criticism & My mental illnesses dictate so much of my daily life that I genuinely don't know what life would be like without them. I've wasted so much of what should have been very formative years for me caught up in being sad or anxious or hating myself all the time that I feel like I never got the chance to develop a personality separate from my illnesses. That makes me terrified of recovery, feeling like my illnesses are a part of me to my very cor \\
% \cmidrule{1-3}
% 1b    & Others' criticism with reason    & I'm in the highway, my dad is driving, he is mad, really mad.He has done this before, but before it was just me, he is treating to kill us, I don't know what to do, I don't want to die like this, I don't want to die by his (obscenity) hands, I'll rather a painful illness that him taking my life, he doesn't deserve my life.Please help, I'm scared.\\
% \cmidrule{1-3}
% 1c    & Others' criticism without reason & First of all  you're all weak. PTSD is a joke. Almost laughable as 9/11 and The Holocaust being real. You're all actors.You're all failures and should've been aborted! You waste of space lame obscenities\{{]}\}. None of you all could ever have your own place cause you're all too slobbish and would be kicked out for your pure incompetence and lack of life.\\                                
% % \cmidrule{1-8}
% % \bottomrule{1-3}
% \bottomrule
% \end{tabular}}
% \caption{Annotations for Criticism}
% \label{criticism_example}
% \end{table}


==> Tables/annotation_intent.tex <==

% \begin{table}[htp]
% \centering
% \begin{tabular}{|p{0.15\textwidth}|p{0.25\textwidth}|p{0.6\textwidth}|}\hline
% Label        & Meaning                                                  & Example                                                                                                                                                                                                                                            \\\hline
% Help-Seeking & OP directly asks for help                                & How do you suppress/repress/get rid of unwanted thoughts that ruminate over and over and over for days upon days upon days and hours upon hours upon hours? I am already in therapy, on meds, with a psychiatrist. It's not working/helping.Thanks \\\hline
% Rant         & OP shares the problem without explicitly asking for help & If I can’t control myself any longer I might just hurt my baby brother one of these days. I can’t take it anymore, and waiting for him to grow up to stop crying is so hard.                                                                       \\\hline
% Survey       & OP asks peers to share their experiences                 & I’m going to be on some meds which will help and with some friends, but still have that deep uncertainty about it all. Crowds, drama, loud noises. How do y’all deal with it?                                                                      \\\hline
% Chitchat     & Small talk, sharing articles/poems etc.                  & Just wanna spread some love and positivity and wish everyone an amazing day that turns into an amazing week that then turns into month and so on. :)                                    \\\hline                                                          
% \end{tabular}
% \caption{Annotations for Intent}
% \label{tab:my-table}
% \end{table}




% \begin{table}[]\centering
% \footnotesize
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|c|p{25em}}
% \toprule
% Label& Meaning&Example\\
% \cmidrule{1-3}
% Help-Seeking & OP directly asks for help                                & How do you suppress/repress/get rid of unwanted thoughts that ruminate over and over and over for days upon days upon days and hours upon hours upon hours? I am already in therapy, on meds, with a psychiatrist. It's not working/helping.Thanks \\
% \cmidrule{1-3}
% Rant         & OP shares the problem without explicitly asking for help & If I can’t control myself any longer I might just hurt my baby brother one of these days. I can’t take it anymore, and waiting for him to grow up to stop crying is so hard.\\
% \cmidrule{1-3}
% Survey       & OP asks peers to share their experiences                 & I’m going to be on some meds which will help and with some friends, but still have that deep uncertainty about it all. Crowds, drama, loud noises. How do y’all deal with it?\\
% \cmidrule{1-3}
% Chitchat     & Small talk, sharing articles/poems etc.                  & Just wanna spread some love and positivity and wish everyone an amazing day that turns into an amazing week that then turns into month and so on. :)\\
% % \cmidrule{1-8}
% % \bottomrule{1-7}
% \bottomrule
% \end{tabular}}
% \caption{Annotation of the intent labels.}
% \label{intent_example}
% \end{table}

\begin{table}[]\centering
\footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{35em}|c|p{10em}}
\toprule
Post & Label & Explanation \\
\cmidrule{1-3}
How do you suppress/repress/get rid of unwanted thoughts that ruminate over and over and over for days upon days upon days and hours upon hours upon hours? I am already in therapy, on meds, with a psychiatrist. It's not working/helping.Thanks & Help-Seeking & User directly asks for help \\
\cmidrule{1-3}
If I can’t control myself any longer I might just hurt my baby brother one of these days. I can’t take it anymore, and waiting for him to grow up to stop crying is so hard. & Rant & User shares the problem without explicitly asking for help\\
\cmidrule{1-3}
I’m going to be on some meds which will help and with some friends, but still have that deep uncertainty about it all. Crowds, drama, loud noises. How do y’all deal with it? & Survey & User asks peers to share their experiences \\
\cmidrule{1-3}
Just wanna spread some love and positivity and wish everyone an amazing day that turns into an amazing week that then turns into month and so on. :) & Chitchat & Small talk, sharing articles/poems etc. \\
% \cmidrule{1-8}
% \bottomrule{1-7}
\bottomrule
\end{tabular}}
\caption{Annotation of the intent labels.}
\label{intent_example}
\end{table}



==> Tables/bodylencomp.tex <==
\begin{table}[htp]
\centering
\begin{tabular}{|l|l|l|l|}\hline
Stat                   & Isolated    & Non interactive & Interactive \\\hline
Min                    & 0           & 0               & 0           \\\hline
Max                    & 4531        & 4416            & 5158        \\\hline
Range                  & 4531        & 4416            & 5158        \\\hline
Distinct               & 483         & 616             & 739         \\\hline
Distinct \%            & 24.8\%      & 16.3\%          & 16.8\%      \\\hline
Mean                   & 154.7170005 & 164.3100981     & 189.9549795 \\\hline
5th percentile         & 0           & 0               & 0           \\\hline
95th percentile        & 532.7       & 538             & 605         \\\hline
Q1                     & 9           & 40              & 53          \\\hline
Q3                     & 192         & 210             & 234         \\\hline
median                 & 86          & 104             & 118         \\\hline
Variance               & 67581.22768 & 47281.93351     & 60380.20084 \\\hline
Standard deviation     & 259.9638969 & 217.4440928     & 245.7238304 \\\hline
CV(coeff of variation) & 1.680254245 & 1.323376319     & 1.293589834 \\\hline
Kurtosis               & 72.50796902 & 68.23817035     & 54.10516306 \\\hline
MAD                    & 86          & 76              & 78          \\\hline
Sum                    & 301234      & 619942          & 835422      \\\hline
Skewness               & 6.41820732  & 5.572602062     & 4.90884295 \\\hline
\end{tabular}
\caption{Comparison of body length stats}
\label{tab:my-table}
\end{table}

==> Tables/commentcomp.tex <==
\begin{table}[htp]
\centering
\begin{tabular}{|l|l|l|}
\hline
Stat                   & Interactive & Non interactive \\\hline
Min                    & 1           & 1               \\\hline
Max                    & 387         & 136             \\\hline
Range                  & 386         & 135             \\\hline
Distinct               & 94          & 49              \\\hline
Distinct \%            & 2.1\%       & 1.3\%           \\\hline
Mean                   & 10.12005457 & 3.418764909     \\\hline
5th percentile         & 2           & 1               \\\hline
95th percentile        & 29          & 10              \\\hline
Q1                     & 4           & 1               \\\hline
Q3                     & 11          & 4               \\\hline
median                 & 6           & 2               \\\hline
Variance               & 210.7251788 & 35.33519391     \\\hline
Standard deviation     & 14.51637623 & 5.944341336     \\\hline
CV(coeff of variation) & 1.434416794 & 1.738739426     \\\hline
Kurtosis               & 151.6912541 & 185.1435227     \\\hline
MAD                    & 3           & 1               \\\hline
Sum                    & 44508       & 12899           \\\hline
Skewness               & 8.931076518 & 11.00225262  \\\hline  
\end{tabular}
\caption{Comparison of number of comments on non-interactive vs interactive posts. (Isolated posts receive 0 comments by definition)}
\label{tab:my-table}
\end{table}

==> Tables/generalstats.tex <==
\begin{table}[htp]

\centering
\scalebox{0.78}{
\begin{tabular}{|l|l|l|l|l|l|}

\hline
Stats & Title Length & Body length & Comments & Unique Posters & Comments by OP \\\hline Zeroes & 0 & 1040 & 1947 & 1947 & 5720 \\\hline
Minimum & 1 & 0 & 0 & 0 & 0 \\\hline
Maximum & 64 & 5158 & 387 & 233 & 79 \\\hline
Range & 63 & 5158 & 387 & 233 & 79 \\\hline

% Mean & 8.67997628   & 173.611188  & 5.673749753    & 3.784937735          & 1.255485274          \\\hline
Mean & 8.67 & 173.61  & 5.67 & 3.78 & 1.25 \\\hline

Median & 7 & 107 & 3 & 2 & 0 \\\hline
Variance & 59.87  & 57086.93  & 121.44 & 42.82 & 7.94 \\\hline
Standard Deviation & 7.73  & 239.92 & 11.02 & 6.54 & 2.81 \\\hline
5th percentile               & 2            & 0           & 0              & 0                    & 0                    \\\hline
95th percentile              & 23           & 569         & 20             & 12                   & 5                    \\\hline
Q1                           & 4            & 41          & 1              & 1                    & 0                    \\\hline
Q3                           & 11           & 217         & 7              & 5                    & 1                    \\\hline
CV(coefficient of variation) & 0.8914901555 & 1.376228838 & 1.942309358    & 1.729022805          & 2.245000444          \\\hline
Kurtosis                     & 10.967       & 63.16400732 & 219.7793746    & 231.5432413          & 144.836085           \\\hline
MAD                          & 3            & 79          & 2              & 2                    & 0                    \\\hline
Skewness                     & 2.763728267  & 5.478783566 & 10.35868289    & 10.76118363          & 8.422516381          \\\hline
Sum                          & 87824        & 1756598     & 57407          & 38296                & 12703   
\\\hline

\end{tabular}
}
\caption{General statistics for the complete data \hl{this will go with a graph. These many stats in one table is not required. Only 2 upto digits required.}}
\label{tab:my-table}

\end{table}

==> Tables/hope_sample.tex <==
% \begin{table}[htp]
% \centering
% \begin{tabular}{|p{0.9\textwidth}|p{0.1\textwidth}|}
% \hline
% Utterance  & Speaker                                         \\ \hline   
% So, Felicity, I think that we've done a lot of good work today. And I'm delighted that you didn't have a panic attack last week. That's really impressive. And you seem really pleased about that as well. And so, you know, I think today we've run through a couple of more techniques that you can use to manage your anxiety. And it seems to me that you've got a good grip on those.                                                                                                                                                   & T    \\ \hline
% Yes. Yeah, definitely. I think today was really helpful.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & P    \\ \hline
% Good. That's fantastic. Well, I guess if we wind up now, and then meet again, next week. Yeah.                                                                                                                                                                                                                                                                                                                                                                                                                                               & T    \\ \hline
% Yeah, yeah. But um, did I did I tell you actually, that I had an argument with my mom on Thursday. Oh, really? Yeah. Yeah. It was a really, really big one. Yeah, I am. Yeah. I mean, what happened was basically that mom, mom, she was just getting really angry at me for Dave again, because you know, we've been going out for three months and it's time I've told you before. Really, really, really doesn't like him.                                                                                                                & P    \\ \hline
% Ohh really?                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & T    \\ \hline
% Yeah. And she was, she had to go in for the drugs again. And then she was saying, you know that I can do so much better. And she was just, you know, like, Oh, I really screaming at me and I had to take all of that and, you know, people were just going around in circles in circles. And it was really, really not not very, not very good that I had listened to her saying that.                                                                                                                                                      & P    \\ \hline
% Yeah, I can imagine so he has been really upset by that.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & T    \\ \hline
% Yeah, I was because, you know, she. Well, you know, that I mean, I really like Dave, I think that is really good. And, and, and, and I would, I would, I would, I would, I would like to keep on seeing him but that she disapproves of him. And I find it really hard. It's just proof of him.                                                                                                                                                                                                                                              & P    \\ \hline
% Yes, I can see that really causes you more anxiety as well that this is happening and yeah, you feel criticized by your mom and perhaps torn a bit between your mom's view and David? Yeah, I do. You talk to him.                                                                                                                                                                                                                                                                                                                           & T    \\ \hline
% While she doesn't, she doesn't want me to talk to him. about it because she doesn't want him to know that she doesn't like him. And then you know, he doesn't really like her as well, because she thinks he thinks that she's a snob. And so it's really hard. You know, I just feel like I'm sort of, sort of in the middle and like in between the two of them. Yeah. But                                                                                                                                                                 & P    \\ \hline
% so felicity. I'm very pleased that you didn't have a panic attack last week. Yeah. And and so are you. Yeah. And I'm hoping that the work that we did today, in looking at a couple more techniques of how you can manage the anxiety has been helpful to you.                                                                                                                                                                                                                                                                               & T    \\ \hline
% Yeah, I think I'll be able to give it a practice this& P    \\ \hline
% week. Good. And we've discussed your homework. Yes. So expert welding perhaps if we wrap up for today.& T    \\ \hline
% All right. What did it do? I tell you that I had an argument with my mom on Thursday.& P    \\ \hline
% No,& T    \\ \hline
% yeah, an argument with mom and it was really bad because she was just yelling, yelling, yelling in your with about Dave. I've told you about Dave before because she doesn't like Dave and she was having a got me for the drug. You know, cuz he takes the drugs and she was just yelling at me because she doesn't like that he takes the drugs, but the student doesn't understand that. I mean, I just want to be with you. And so but because she doesn't like him see, you know, sister, she was yelling at me about that on Thursday, & P    \\
% I can see that this is very upsetting for you. felicitated is an issue that you've raised before. So I'm wondering whether we should decide that for next week, we'll start to discuss these issues that you're having with your mom so that we can work out a plan when we've got our next session. How would that be? & T   
% \\ 
% \hline
% \end{tabular}
% \caption{A sample conversation from the HOPE dataset. Here, T denotes utterances from the therapist, and P denotes the help-seeker)}
% \end{table}




\begin{table}[]\centering
% \footnotesize
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{50em}|c}\toprule

Utterance  & Speaker\\ 
\toprule  
So, Felicity, I think that we've done a lot of good work today. And I'm delighted that you didn't have a panic attack last week. That's  impressive. And you seem really pleased about that as well. So, you know, I think today we've run through a couple of more techniques that you can use to manage your anxiety. And you've got a good grip on those.& Therapist    \\ \cmidrule{1-2}
Yes. Yeah, definitely. I think today was really helpful.& Client    \\ \cmidrule{1-2}
Good. That's fantastic. Well, I guess if we wind up now, and then meet again, next week. Yeah.& Therapist    \\ \cmidrule{1-2}
Yeah, yeah. But um, did I did I tell you actually, that I had an argument with my mom on Thursday. Oh, really? Yeah. Yeah. It was a really, really big one. Yeah, I am. Yeah. I mean, what happened was basically that mom, mom, she was just getting really angry at me for Dave again, because you know, we've been going out for three months and it's time I've told you before. Really, really, really doesn't like him.& Client    \\ \cmidrule{1-2}
Ohh really?& Therapist    \\ \cmidrule{1-2}
Yeah. And she was, she had to go in for the drugs again. And then she was saying, you know that I can do so much better. And she was just, you know, like, Oh, I really screaming at me and I had to take all of that and, you know, people were just going around in circles in circles. And it was really, really not not very, not very good that I had listened to her saying that.& Client    \\ \cmidrule{1-2}
Yeah, I can imagine so he has been really upset by that.& Therapist    \\ \cmidrule{1-2}
Yeah, I was because, you know, she. Well, you know, that I mean, I really like Dave, I think that is really good. And, and, and, and I would, I would, I would, I would, I would like to keep on seeing him but that she disapproves of him. And I find it really hard. It's just proof of him.& Client    \\ \cmidrule{1-2}
Yes, I can see that really causes you more anxiety as well that this is happening and yeah, you feel criticized by your mom and perhaps torn a bit between your mom's view and David? Yeah, I do. You talk to him.& Therapist  \\ \cmidrule{1-2}
While she doesn't, she doesn't want me to talk to him. about it because she doesn't want him to know that she doesn't like him. And then you know, he doesn't really like her as well, because she thinks he thinks that she's a snob. And so it's really hard. You know, I just feel like I'm sort of, sort of in the middle and like in between the two of them. Yeah. But so felicity. & Client    \\ \cmidrule{1-2}
I'm very pleased that you didn't have a panic attack last week. Yeah. And so are you. And I'm hoping that the work that we did today, in looking at a couple more techniques of how you can manage the anxiety has been helpful to you.& Therapist    \\ \cmidrule{1-2}
% Yeah, I think I'll be able to give it a practice this week. & Client    \\ \cmidrule{1-2}
% Good. And we've discussed your homework. Yes. So expert welding perhaps if we wrap up for today.& Therapist    \\ \cmidrule{1-2}
% All right. What did it do? I tell you that I had an argument with my mom on Thursday.& Client    \\ \cmidrule{1-2}
% No,& Therapist    
... & ...
\\ \cmidrule{1-2}
yeah, an argument with mom and it was really bad because she was just yelling, yelling, yelling in your with about Dave. I've told you about Dave before because she doesn't like Dave and she was having a got me for the drug. You know, cuz he takes the drugs and she was just yelling at me because she doesn't like that he takes the drugs, but the student doesn't understand that. I mean, I just want to be with you. And so but because she doesn't like him see, you know, sister, she was yelling at me about that on Thursday, & Client    \\
\cmidrule{1-2}

I can see that this is very upsetting for you. felicitated is an issue that you've raised before. So I'm wondering whether we should decide that for next week, we'll start to discuss these issues that you're having with your mom so that we can work out a plan when we've got our next session. How would that be? & Therapist 
\\
\bottomrule
\multicolumn{2}{c}{} \\
\end{tabular}}
\caption{A sample conversation from the HOPE dataset. Here the conversation is between therapist and client (aka help-seeker). }
\label{tab:HOPE_example}
\end{table}


==> Tables/peerData.tex <==
\begin{table}[]\centering
\footnotesize
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c|c|p{25em}}
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\begin{tabular}{l|cc|cccc|cccc|cc}
\toprule
\multirow{3}{*}{\bf Subreddits} & \multirow{3}{*}{\bf Posts} & \multirow{3}{*}{\bf Comments} & \multicolumn{4}{c|}{\bf Intent} & \multicolumn{4}{c|}{\bf Criticism} & \multicolumn{2}{c}{\bf Readability}\\
\cmidrule{4-13}
&&& \multirow{2}{4em}{\centering \textbf{Help seeking}} & \multirow{2}{*}{\textbf{Rant}} & \multirow{2}{*}{\textbf{Survey}} & \multirow{2}{*}{\textbf{Chitchat}} & 	\multirow{2}{4em}{\centering \textbf{Self criticism}} & 	\multirow{2}{4em}{\centering \textbf{Other w/ Reason}}  & 	\multirow{2}{5em}{\centering \textbf{Other w/o Reason}}& 	\multirow{2}{4em}{\centering \textbf{No criticism}} & \multirow{2}{*}{\textbf{Clear}}  & \multirow{2}{*}{\textbf{Non-clear}} \\
% \cmidrule{1-13}
& & & & & & & & & & & & \\
\cmidrule{1-13}

% r/Anxiety &	469 & 1773 & 252 & 129 & 62 & 26 & 278 & 48 & 7 & 136 & 467 & 2\\
% % \cmidrule{1-13}
% r/ptsd	&	494	&	1567	&	221	&	144	&	64	&	65	&	180	&	135	&	1	&	178	&	494	&	0\\
% % \cmidrule{1-13}
% r/suicideWatch	&	403	&	2545	&	90	&	246	&	17	&	50	&	231	&	34	&	10	&	128	&	378	&	25\\
% % \cmidrule{1-13}
% r/addiction	&	487	&	3581	&	217	&	148	&	43	&	79	&	246	&	67	&	6	&	168	&	466	&	21\\
% % \cmidrule{1-13}
% r/ADHD	&	423	&	3856	&	169	&	104	&	78	&	72	&	139	&	31	&	9	&	247	&	418	&	5\\
% % \cmidrule{1-13}
% r/alcoholicsanonymous	&	498	&	6021	&	181	&	107	&	47	&	163	&	155	&	58	&	5	&	280	&	490	&	8\\
% % \cmidrule{1-13}
% r/Anger	&	464	&	2620	&	233	&	184	&	31	&	16	&	245	&	140	&	16	&	63	&	462	&	2\\
% % \cmidrule{1-13}
% r/BPD	&	519	&	2744	&	180	&	185	&	113	&	41	&	234	&	99	&	4	&	182	&	518	&	1\\
% % \cmidrule{1-13}
% r/depression	&	547	&	1951	&	83	&	363	&	26	&	75	&	243	&	91	&	18	&	195	&	546	&	1\\
% % \cmidrule{1-13}
% r/domesticviolence	&	425	&	2847	&	254	&	94	&	25	&	52	&	34	&	277	&	1	&	113	&	421	&	4\\
% % \cmidrule{1-13}
% r/eating\_disorders	&	568	&	2021	&	256	&	209	&	51	&	52	&	346	&	43	&	1	&	178	&	567	&	1\\
% % \cmidrule{1-13}
% r/getting\_over\_it	&	476	&	2551	&	230	&	163	&	35	&	48	&	258	&	72	&	2	&	144	&	473	&	3\\
% % \cmidrule{1-13}
% r/mentalillness	&	484	&	1895	&	208	&	155	&	52	&	69	&	209	&	99	&	2	&	174	&	480	&	4\\
% % \cmidrule{1-13}
% r/OpiatesRecovery	&	493	&	6112	&	215	&	116	&	62	&	100	&	185	&	28	&	3	&	277	&	493	&	0\\
% % \cmidrule{1-13}
% r/rapecounseling	&	481	&	2390	&	288	&	142	&	26	&	25	&	125	&	269	&	1	&	86	&	481	&	0\\
% % \cmidrule{1-13}
% r/sad	&	486	&	2258	&	44	&	287	&	27	&	128	&	115	&	71	&	8	&	292	&	485	&	1\\
% % \cmidrule{1-13}
% r/selfharm	&	467	&	1928	&	136	&	232	&	52	&	47	&	243	&	39	&	0	&	185	&	465	&	2\\
% % \cmidrule{1-13}
% r/selfhelp	&	419	&	2001	&	177	&	60	&	28	&	154	&	163	&	37	&	0	&	219	&	390	&	29\\
% % \cmidrule{1-13}
% r/socialanxiety	&	461	&	2798	&	167	&	128	&	64	&	102	&	201	&	58	&	0	&	202	&	428	&	33\\

% r/OCD	&	424	&	2528	&	159	&	117	&	63	&	85	&	209	&	29	&	3	&	183	&	424	&	0\\
% r/helpmecope	&	473	&	2121	&	277	&	127	&	17	&	52	&	170	&	160	&	2	&	141	&	471	&	2\\

% \toprule

\bf 21	&	\bf9961	&	\bf58108	&	\bf4037	&	\bf3440	&	\bf983	&	\bf1501	&	\bf4209	&	\bf1885	&	\bf99	&	\bf3771	&	\bf9817	&	\bf144\\

\cmidrule{1-13}
\rowcolor{yellow!20}
\bf IAA	($\kappa$)&-&-&	\multicolumn{4}{c|}{\bf 0.963} & \multicolumn{4}{c|}{\bf 0.888}& \multicolumn{2}{c}{\bf 0.861}\\
\bottomrule

\end{tabular}}
\caption{The table shows the statistics of the \peerData. We collect a total of $\sim10K$ posts and $\sim50K$ comments. We annotate all the posts for three core labels a) intent, b) criticism, and c) readability [Clear: Excellent, Good and Average; Non-clear: Mediocre and Poor]. IAA ($\kappa$) represents the Inter-Annotator Agreement using Cohen's kappa score.}
\label{tab:peerDataStats}
\end{table}

==> Tables/peercoms.tex <==
\begin{table}[htp]
\centering
\begin{tabular}{|l|l|l|}
\hline
Stat                   & Interactive & Non interactive \\\hline
Min                    & 0           & 1               \\\hline
Max                    & 382         & 136             \\\hline
Range                  & 382         & 135             \\\hline
Distinct               & 85          & 49              \\\hline
Distinct \%            & 1.9\%       & 1.3\%           \\\hline
Mean                   & 7.231696226 & 3.418764909     \\\hline
5th percentile         & 1           & 1               \\\hline
95th percentile        & 22          & 10              \\\hline
Q1                     & 4           & 1               \\\hline
Q3                     & 11          & 4               \\\hline
median                 & 4           & 2               \\\hline
Variance               & 155.7118266 & 35.33519391     \\\hline
Standard deviation     & 12.4784545  & 5.944341336     \\\hline
CV(coeff of variation) & 1.725522492 & 1.738739426     \\\hline
Kurtosis               & 251.0875205 & 185.1435227     \\\hline
MAD                    & 2           & 1               \\\hline
Sum                    & 31805       & 12899           \\\hline
Skewness               & 11.68860524 & 11.00225262 \\\hline   
\end{tabular}
\caption{Number of comments other than those by original poster(peers).}
\label{tab:my-table}
\end{table}

==> Tables/postercomp.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
Stat                   & Interactive & Non interactive \\\hline
Min                    & 1           & 1               \\\hline
Max                    & 233         & 104             \\\hline
Range                  & 232         & 103             \\\hline
Distinct               & 65          & 41              \\\hline
Distinct \%            & 1.5\%       & 1.1\%           \\\hline
Mean                   & 6.075943611 & 3.067585476     \\\hline
5th percentile         & 2           & 1               \\\hline
95th percentile        & 17          & 9               \\\hline
Q1                     & 3           & 1               \\\hline
Q3                     & 7           & 3               \\\hline
median                 & 4           & 2               \\\hline
Variance               & 68.99400383 & 20.41298136     \\\hline
Standard deviation     & 8.306262928 & 4.518072749     \\\hline
CV(coeff of variation) & 1.367073735 & 1.472843311     \\\hline
Kurtosis               & 182.620485  & 147.953178      \\\hline
MAD                    & 2           & 1               \\\hline
Sum                    & 26722       & 11574           \\\hline
Skewness               & 10.05613717 & 9.530456343    \\\hline
\end{tabular}
\caption{Comparison of interactive and non interactive posts based on unique number of comment posters.}
\label{tab:my-table}
\end{table}

==> Tables/subtable.tex <==
\begin{table}[htp]
\begin{adjustbox}{width=\textwidth,center=\textwidth}
\begin{tabular}{|l|c|c|c|c|l|}
\hline
Sub-reddit            & No of Subscribers & No of Posts Collected & No of Comments Collected & Start Date & End Date   \\
\hline
r/ptsd                & 66.1k             & 500                   & 2995                     & 01/01/2020 & 21/01/2020 \\
\hline
r/ADHD                & 1.3million        & 500                   & 3856                     & 01/01/2020 & 04/01/2020 \\
\hline
r/OCD                 & 132k              & 500                   & 2528                     & 01/01/2020 & 08/01/2020 \\
\hline
r/alcoholicsanonymous & 39.2k             & 500                   & 6021                     & 01/01/2020 & 04/02/2020 \\
\hline
r/Anxiety             & 496k              & 500                   & 1773                     & 01/01/2020 & 03/01/2020 \\
\hline
r/mentalillness       & 104k              & 500                   & 1895                     & 01/01/2020 & 27/01/2020 \\
\hline
r/addiction           & 60.5k             & 500                   & 3581                     & 01/01/2020 & 26/01/2020 \\
\hline
r/socialanxiety       & 316k              & 500                   & 2798                     & 01/01/2020 & 09/01/2020 \\
\hline
r/selfharm            & 82.4k             & 500                   & 1928                     & 01/01/2020 & 06/01/2020 \\
\hline
r/depression          & 806k              & 500                   & 1951                     & 01/01/2020 & 01/01/2020 \\
\hline
r/domesticviolence    & 17.4k             & 500                   & 2847                     & 01/01/2020 & 17/03/2020 \\
\hline
r/eating\_disorders   & 13k               & 599                   & 2021                     & 01/01/2020 & 06/06/2020 \\
\hline
r/rapecounselling     & 21.8k             & 599                   & 2390                     & 01/01/2020 & 19/03/2020 \\
\hline
r/BPD                 & 155k              & 599                   & 2744                     & 01/01/2020 & 06/01/2020 \\
\hline
r/SuicideWatch        & 313k              & 500                   & 2352                     & 01/01/2020 & 04/02/2020 \\
\hline
r/OpiatesRecovery     & 34.1k             & 500                   & 6112                     & 01/01/2020 & 05/02/2020 \\
\hline
r/getting\_over\_it   & 32k               & 500                   & 2551                     & 01/01/2020 & 05/06/2020 \\
\hline
r/Anger               & 30k               & 500                   & 2620                     & 01/01/2020 & 25/03/2020 \\
\hline
r/helpmecope          & 6.3k              & 500                   & 2120                     & 01/01/2020 & 20/05/2020 \\
\hline
r/sad                 & 116k              & 500                   & 2258                     & 01/01/2020 & 15/01/2020 \\
\hline
r/selfhelp            & 142k              & 500                   & 2001                     & 01/01/2020 & 10/02/2020 \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Information about Sub-Reddits scraped}
\end{table}



==> Tables/titlelengthcomp.tex <==
\begin{table}[htp]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Stat                   & Isolated     & Non interactive & Interactive  \\\hline
Min                    & 1            & 1               & 1            \\\hline
Max                    & 61           & 64              & 64           \\\hline
Range                  & 60           & 63              & 63           \\\hline
Distinct               & 55           & 58              & 62           \\\hline
Distinct \%            & 2.8\%        & 1.5\%           & 1.4\%        \\\hline
Mean                   & 8.798151002  & 8.477604029     & 8.801273306  \\\hline
5th percentile         & 1            & 2               & 2            \\\hline
95th percentile        & 24           & 22              & 23           \\\hline
Q1                     & 4            & 4               & 4            \\\hline
Q3                     & 11           & 11              & 11           \\\hline
median                 & 6            & 7               & 7            \\\hline
Variance               & 69.23415896  & 53.49823901     & 61.18224082  \\\hline
Standard deviation     & 8.320706638  & 7.314249039     & 7.821907748  \\\hline
CV(coeff of variation) & 0.9457335566 & 0.862773139     & 0.8887245602 \\\hline
Kurtosis               & 10.4901406   & 11.75495108     & 10.43530091  \\\hline
MAD                    & 3            & 3               & 3            \\\hline
Sum                    & 17130        & 31986           & 38708        \\\hline
Skewness               & 2.77648661   & 2.805000425     & 2.701711219 \\
\hline
\end{tabular}
\caption{Comparison of title length stats}
\label{tab:my-table}
\end{table}
